Discrete quantitative Helly-type theorems with boxes

Research on Helly-type theorems in combinatorial convex geometry has produced volumetric versions of Helly's theorem using witness sets and quantitative extensions of Doignon's theorem. This paper combines these philosophies and presents quantitative Helly-type theorems for the integer lattice with axis-parallel boxes as witness sets. Our main result shows that, while quantitative Helly numbers for the integer lattice grow polynomially in each fixed dimension, their variants with boxes as witness sets are uniformly bounded. We prove several colorful and fractional variations on this theorem. We also prove that the Helly number for $A \times A \subseteq \mathbb{R}^2$ need not be finite even when $A \subseteq \mathbb{Z}$ is a syndetic set.

==> extras.tex <==
% Proposition 2.19:

The function
\[  f(x,y) = \begin{cases}
        \prod\limits_{i=1}^d (y_i - x_i + 1) &\text{if } \min_i \{y_i - x_i\} \geq t \\
        \ 0 &\text{otherwise,}
    \end{cases} \]
is min-concave on the set of boxes. If $\bx(x,y)$ is $t$-thick and contains at least $n$ lattice points, then $f(x,y) \geq n$. Applying \cref{thm:box-weighting-min-concave} (and the mixed-integer Helly theorem) to $\mathcal F$ with $S = \Z^d$ and $T = \R^m \times \Z^{d-m}$ provides a point $(a,b) \in \Z^d \times (\R^m \times \Z^{d-m})$ with 
$\bx(a,b) \subseteq \bigcap \mathcal F$ and $f(a,b) \geq n$. Thus, $\bx(a,b)$ is $t$-thick and contains
\[  \prod_{i=1}^m\lfloor b_i - a_i + 1\rfloor\prod_{i=m+1}^{d} (b_i - a_i + 1)\]
lattice points. Using the substitution $y_i = b_i - a_i + 1$, the product is bounded below by
\[
    \min \left\{ \prod_{i=1}^m \lfloor y_i \rfloor\prod_{i=m+1}^d y_i\, :\, y_i \geq t+1 \text{ and } \prod_{i=1}^d y_i = n \right\}.
\]
which in turn has a lower bound of
\begin{align*}
    &\min\left\{\prod_{i=1}^d y_i\, :\, y_i \geq \lfloor t\rfloor + 1 \text{ and } \prod_{i=1}^m (y_i+1)\prod_{i=m+1}^d y_i \geq n \right\}\\
    = &\min\left\{\prod_{i=1}^d y_i\, :\, y_i \geq \lfloor t\rfloor + 1 \text{ and } \prod_{i=1}^m (y_i+1)\prod_{i=m+1}^d y_i = n \right\}.
\end{align*}
Using the product condition on the right, we have
\[ 
    \prod_{i=1}^d y_i = n\, \prod_{i=1}^m\! \left(\frac{y_i}{y_i+1}\right),
\]
so this minimum is at least
\[
    \min\left\{n\, \prod_{i=1}^m\! \left(\frac{y_i}{y_i+1}\right)\, :\, y_i \geq \lfloor t\rfloor + 1 \text{ and } \prod_{i=1}^m (y_i+1) \leq n \right\}.
\]
This final minimum is achieved when $y_i = \lfloor t\rfloor + 1$ for every $1 \leq i \leq d$, and its value is
\[
    \frac{n}{\left(1+\frac{1}{\lfloor t\rfloor + 1}\right)^m}.\qedhere
\]





% Proposition 2.20:

The proof is similar to that of \cref{thm:lower-Helly-number1}. We apply \cref{thm:box-weighting-min-concave} to $\mathcal F$ with the same function $f$ and $S = \R^m \times \Z^{d-m}$ and $T = \R^d$ to get a point $(a,b) \in (\R^m \times \Z^{d-m}) \times \R^d$ such that $\bx(a,b) \subseteq \bigcap \mathcal F$ and $f(a,b) \geq n$. The set $\bx(a,b)$ contains at least
\[  \prod_{i=1}^m \lfloor b_i - a_i\rfloor \prod_{i=m+1}^{d} \lfloor b_i-a_i + 1\rfloor \]
lattice points. Substituting $y_i = b_i - a_i$, this product is bounded below by 
\begin{align*}
    &\min\left\{ \prod_{i=1}^m \lfloor y_i\rfloor\prod_{i=m+1}^{d} \lfloor y_i + 1\rfloor\,
        :\, y_i \geq t \text{ and } \prod_{i=1}^d (y_i+1) = n \right\} \\
    \geq &\min\left\{\prod_{i=1}^d y_i\,
        :\, y_i \geq \lfloor t\rfloor \text{ and } \prod_{i=1}^m (y_i+2)\prod_{i=m+1}^{d} (y_i+1) = n \right\}.
\end{align*}

Using the right-hand product condition, this minimum is equal to
\[
    \min\left\{n\, \prod_{i=1}^m \left(\frac{y_i}{y_i+2}\right) \prod_{i=m+1}^d\!\left(\frac{y_i}{y_i+1}\right)\,
        :\, y_i \geq \lfloor t\rfloor \text{ and } \prod_{i=1}^m (y_i+2)\prod_{i=m+1}^{d} (y_i+1) = n \right\}.
\]
Setting $y_i = \lfloor t\rfloor$ for every $1 \leq i \leq d$ bounds this minimum below by
\[
    \frac{n}{\left(1 + \frac{1}{\lfloor t\rfloor}\right)^{d-m}
             \left(1 + \frac{2}{\lfloor t\rfloor}\right)^m}.\qedhere
\]
